The Muon Smasher's Guide

We lay out a comprehensive physics case for a future high-energy muon collider, exploring a range of collision energies (from 1 to 100 TeV) and luminosities. We highlight the advantages of such a collider over proposed alternatives. We show how one can leverage both the point-like nature of the muons themselves as well as the cloud of electroweak radiation that surrounds the beam to blur the dichotomy between energy and precision in the search for new physics. The physics case is buttressed by a range of studies with applications to electroweak symmetry breaking, dark matter, and the naturalness of the weak scale. Furthermore, we make sharp connections with complementary experiments that are probing new physics effects using electric dipole moments, flavor violation, and gravitational waves. An extensive appendix provides cross section predictions as a function of the center-of-mass energy for many canonical simplified models.

==> higgscouplings.tex <==

\begin{table}[t]
\renewcommand{\arraystretch}{1.5}
\setlength{\arrayrulewidth}{.3mm}
\setlength{\tabcolsep}{0.8 em}
\begin{center}
\begin{tabular}{c|c|c|c|c} %\hline
\multicolumn{5}{c}{10 TeV @ $10\,\textrm{ab}^{-1}$} \\ \hline
Production & Decay & Rate [fb] & $A \cdot \epsilon$ [\%] & $\Delta \sigma / \sigma$ [\%] \\ \hline \hline
\multirow{12}{*}{$W$-fusion} & $bb$ & $485.7$ & 7.4 & 0.17 \\ \cline{2-5} 
 & $cc$ & $24.4$ & 1.4 & 1.71 \\ \cline{2-5} 
 & $jj$ & $72.1$ & 37.2 & 0.19 \\ \cline{2-5} 
 & $\tau^+ \tau^-$ & $53.1$ & 6.5 & 0.54 \\ \cline{2-5} 
 & $WW^*(jj\ell\nu)$ & $52.8$ & 20.7 & 0.30 \\ \cline{2-5} 
 & $WW^*(4j)$ & $85.7$ & 4.9 & 0.49 \\ \cline{2-5} 
 & $ZZ^*(4\ell)$ & $0.1$ & 6.6 & 11.74 \\ \cline{2-5} 
 & $ZZ^*(jj\ell^+\ell^-)$ & $2.1$ & 8.9 & 2.32 \\ \cline{2-5} 
 & $ZZ^*(4j)$ & $10.8$ & 4.6 & 1.42 \\ \cline{2-5} 
 & $\gamma\gamma$ & 1.9 & 33.0 & 1.25 \\ \cline{2-5} 
 & $Z(jj)\gamma$ & $0.9$ & 27.2 & 1.99 \\ \cline{2-5} 
 & $\mu^+ \mu^-$ & $0.2$ & 36.7 & 0.37 \\ \hline
\multirow{2}{*}{$Z$-fusion} & $bb$ & 50.6 & 8.1 & 0.49 \\ \cline{2-5} 
 & $WW^*(4j)$ & 8.9 & 6.2 & 1.34 \\ \hline
$ttH$ & $bb$ & $0.05$ & 8.6 & 14.95 \\ \hline
\end{tabular}
\end{center}
\caption{
Signal rates and efficiencies for selected Higgs production channels at a $10\,\textrm{TeV}$ muon collider. \textcolor{blue}{SH: More details..}
}\label{tab:higgsrateprecision}
\end{table}





\begin{table}[t]
\renewcommand{\arraystretch}{1.5}
\setlength{\arrayrulewidth}{.3mm}
\setlength{\tabcolsep}{0.8 em}
\begin{center}
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{Fit Result [\%]} \\ \hline
 & \multicolumn{1}{c|}{$10\,\textrm{TeV}$ Muon Collider} & \multicolumn{1}{c|}{with HL-LHC} & with HL-LHC + $250\,\textrm{GeV}$ $e^+e^-$ \\ \hline \hline
$\kappa_W$ & 0.06 & 0.06 & 0.06 \\ \hline
$\kappa_Z$ & 0.23 & 0.22 & 0.10 \\ \hline
$\kappa_g$ & 0.15 & 0.15 & 0.15 \\ \hline
$\kappa_{\gamma}$ & 0.64 & 0.57 & 0.57 \\ \hline
$\kappa_{Z\gamma}$ & 1.00 & 1.00 & 0.97 \\ \hline
$\kappa_c$ & 0.89 & 0.89 & 0.79 \\ \hline
$\kappa_t$ & 7.49 & 2.94 & 2.94 \\ \hline
$\kappa_b$ & 0.16 & 0.16 & 0.15 \\ \hline
$\kappa_{\mu}$ & 1.95 & 1.80 & 1.76 \\ \hline
$\kappa_{\tau}$ & 0.31 & 0.30 & 0.27 \\ \hline
\end{tabular}
\end{center}
\caption{
Results of a 10-parameter fit to the Higgs couplings in the $\kappa$-framework, based on the attainable precision in each production and decay channel listed in Table~\ref{tab:higgsrateprecision}. \textcolor{blue}{SH: More details...}
}\label{tab:higgscouplingfit}
\end{table}

